Recommending API Function Calls and Code Snippets to Support Software Development

Software development activity has reached a high degree of complexity, guided by the heterogeneity of the components, data sources, and tasks. The proliferation of open-source software (OSS) repositories has stressed the need to reuse available software artifacts efficiently. To this aim, it is necessary to explore approaches to mine data from software repositories and leverage it to produce helpful recommendations. We designed and implemented FOCUS as a novel approach to provide developers with API calls and source code while they are programming. The system works on the basis of a context-aware collaborative filtering technique to extract API usages from OSS projects. In this work, we show the suitability of FOCUS for Android programming by evaluating it on a dataset of 2,600 mobile apps. The empirical evaluation results show that our approach outperforms two state-of-the-art API recommenders, UP-Miner and PAM, in terms of prediction accuracy. We also point out that there is no significant relationship between the categories for apps defined in Google Play and their API usages. Finally, we show that participants of a user study positively perceive the API and source code recommended by FOCUS as relevant to the current development context.

==> src/Threats.tex <==
The main threat to {\em construct validity} concerns the simulated setting used to evaluate the approaches, as opposed to performing a user study. We mitigated this threat by introducing four configurations that simulate different stages of the development process. In a real development setting, however, the order in which one writes statements might not fully reflect our simulation. Also, in a real setting, there may be cases in which a recommender is more useful, and cases (obvious code completion) where it is less useful.  This makes a further evaluation involving developers highly desirable.

Threats to {\em internal validity} concern factors internal to our study that could have influenced the results. One possible threat can be seen through the results obtained for the datasets \code{SH$_L$} and \code{SH$_S$}. As noted, these datasets exhibit lower precision/recall with respect to \code{MV$_L$} and \code{MV$_S$} due to the limited size of the training sets. However, these datasets were needed to compare FOCUS and PAM due to the limited scalability of PAM.
%such datasets, and in particular \code{SH$_S$}, were created to allow us to compare FOCUS with PAM, otherwise less feasible on larger datasets.

The main threat to {\em external validity} is that FOCUS is currently limited to Java programs.
%is currently limited to Java programs, though in principle the approach could be implemented and evaluated with other programming languages.
As stated in \Cref{sec:ProposedApproach}, however, FOCUS makes few assumptions on the underlying language and only requires information about method declarations and invocations to build the 3D rating matrix. This information could be extracted from programs written in any object-oriented programming language, and we wish to generalize FOCUS to other languages in the future.

